The PUEVA Inventory: A Toolkit to Evaluate the Personality, Usability and Enjoyability of Voice Agents

The proliferation of voice agents in consumer devices requires new tools for evaluating these systems beyond their technical functionality. This paper presents a toolkit for the evaluation of Voice User Interfaces (VUIs) with the intention of measuring the crucial factors of subjective enjoyment in the user experience. The PUEVA toolkit was constructed using a meta-analysis of existing literature, structured N=20 and semi-structured N=18 interviews and a within subjects lab study. The resulting questionnaire contains 35 items that represent 12 scales in three categories: (1) Personality (2) Usablity and (3) Enjoyability. The PUEVA Toolkit moves us towards the capacity to evaluate and compare subjective, joyful experiences in between-subject as well as within-subject research designs.

==> 01intro.tex <==
\section{Introduction}
Voice agents which interact via natural speech input and respond using a synthesised voice are commonly found in mobile phones and home speakers. Recently, voice agents have made significant inroads into homes, offices and automobiles \cite{corbett2016can}. The growth in the medium of voice agents for interaction argues for the development of new tools and techniques for the design and evaluation of those interactions. As natural language generation (NLG) has improved, voice agents have been imparted with additional personality traits expanding interaction beyond the mechanized style of earlier voice agents\cite{chen2010behavior}. More expansive interactive capacity necessitates new tools for the design and development of interactive agents.

Creating a voice agent requires focusing on features of use that extend beyond bare utility and aesthetic. Voice user agents are avatars that are imbued with human traits and characteristics. The characterization of VUIs manifests in the speech tone and prosody of the agents, as well as the content of an interaction. The combined effect of these features is to shape an assistant that may enable a more enjoyable interaction  for users. 

Given the number of new applications that use voice agents as an interface, we felt that the community needed a common toolkit for evaluating the perceived enjoyment and user experience of interactions with voice agents, one that could be used across different voice agent applications. Few studies exist on what people do to overcome VUI problems they encounter. In this paper, we present the design of an inventory questionnaire intended to help designers and researchers working on novel voice user agents to evaluate their designs. The scales that currently exist do not completely capture a user’s experience with VUIs. Moreover, the importance of specific aspects of existing scales may have changed. Our new scale respects prior academic work by building on previous scales, and makes it easier to compare systems evaluated with older scales with future systems evaluated using our scale. We drew on existing literature and existing scales to test a super-set of current scales, and used principal component analysis to reduce these to a more practicable toolkit of questions.


==> 02related_work.tex <==
\section{Related work}
\subsection{Voice User Interfaces}
While there are pragmatic reasons for the increase of voice interfaces on a variety of consumer devices, the ubiquity of voice user agents is often related to the desire to make for more ``natural'' user experiences  \cite{castelluccio2019conversational}. \citet{reeves2018not} point out that voice agents are often called ``conversational agents,'' but the technology, to date, is not actually conversational, so it is not clear that metrics that are used to evaluate conversation are appropriate for these technologies. Interviews and surveys with people comparing qualities of good human conversation with good human-agent conversation indicate that people evaluate human conversations around relationship building and maintenance, but have more transactional standards around interactions with voice agents. \cite{clark2019makes} 

That said, a substantial body of prior research on voice user interfaces indicate that factors beyond mere task execution color the experience and enjoyment people have interacting with a voice agent. \citet{nass2001does}, for example, showed how users ascribe personality to computer synthesized voices, even in very simple applications, which can be leveraged to design for likability and agent trust. When evaluating a WoZ voice agent prototype that responded only to polite requests, researchers asked questions regarding emotional affect and efficiency of such an agent \cite{bonfert2018if}. Users expressed a need for a interaction efficiency, but also preferred one with personality so long as it did not hinder that efficiency. As \citet{nass2005wired} point out, interactive technologies are capable of triggering our natural social responses to speech \cite{nass2005wired} which necessitate tools that allow for evaluation along dimensions of both usability and personality.

While numerous studies exist evaluating the usability and user experience of a variety of VUIs \cite{abdolrahmani2018siri, pyae2018investigating, lopez2017alexa, ehrenbrink2017google}, often for different populations or domains \cite{lovato2015siri,corbett2016can, mennicken2018challenges, sayago2019voice, pal2019user, kowalski2019older,augstein2019weldvui}, these evaluations are often difficult to compare or cross apply because they use different measures and scales to evaluate the interactions. Developing and leveraging a more standardized questionnaire that captures both usability and personality would allow for cross-context VUI prototype evaluation, comparison and the development of design best practices for voice agents. 

\subsection{Evaluation as Part of Voice User Interface Design}

Many of the HCI studies performed on existing consumer voice interfaces are executed by academics after a product is shipping, but, from the perspective of this paper's authors, the most useful phase of the product life cycle in which to perform evaluation is when interactions are being authored. This point-of-view argues for a lightweight and flexible evaluation tool that allows people to compare different platforms \textit{(Should we build use Cortana or Google Voice for this automotive application?)}, different use cases \textit{(Does this voice application work as well in English as it does in Japanese?)}, different voices \textit{(Should we use a male or a female voice for this?)}\cite{cambre2020choice} or different interaction designs \textit{(Should we make our voice agent more polite, or more assertive?)} around common subjective factors. %While some aspects of VUIs, such as the choice of voices, are inherent to the platform they are deployed on, such as Siri Shortcuts (Apple), Alexa Skills (Amazon) and and Voice Actions (Google), others may have much to do with the specific interactions and responses created by developers using these platforms' software development kits (SDK). 

At each stage of prototyping, VUIs must be evaluated while accounting for the conversational interaction paradigm.\cite {murad2019revolution}   %The novelty of ubiquitous VUIs corresponds with a shortage in sufficient design heuristics and pedagogical tools
\citet{wei2018evaluating} and \citet{murad2019tools} have proffered useful heuristics as guidelines for designing voice user interfaces. These tools are useful to designers of speech-based interfaces because they are specific to VUIs, as opposed to GUIs. Social acceptance, for example is not a typical metric for users interacting with a GUI, whereas it is a critical measure for speech and gesture based interfaces which may be used in public settings \cite{rico2010gesture}. While usability heuristics are useful as guidelines, %for design scenarios which can easily be observed and study by usability evaluators, 
 we believe VUIs to be more like mobile apps, which tend to want to be studied in the context where they are used, or webpages, which are easily deployed at scale. Therefore, we believe a questionnaire-based evaluation tool, wherein the users are asked to self-evaluate the qualitative aspects of the voice agent following an actual interaction with the system, are more appropriate than heuristic-based tools for making key design decisions.

\subsection{Questionnaires for Usability, UX and Interaction}
%Questionnaires are commonly used in HCI to evaluate user interfaces and novel applications. 
While novel interfaces or systems sometimes require bespoke evaluation instruments intended to ensure that the designed system fulfills its intended purpose, early HCI researchers found that it was useful to develop standardized evaluation instruments to measure different software with a common yardstick.   \citet{chin1988Development}, for instance, developed the Questionnaire for User Interface Satisfaction in 1988; the questions on the interface focused on the user's response to their use of software, rather than on aspects of the software itself, enabling the same tool to be used to measure command line systems and menu-driven applications, with a high degree of reliability. Other early questionnaires included IBM's After-Scenario Questionnaire (ASQ) \cite{lewis1995ibm} and the Post-Study System Usability Questionnaire (PSSUQ) \cite{lewis1992psychometric}. 

While these early instruments all had strong internal consistency, they often focused on user's self assessment of task completion and satisfaction, and often were not sensitive enough to pick up on the effects of various design changes \cite{hornbaek2006current}. Later questionnaires broadened to consider adaptation to other contexts (for example, educational technology \cite{harrati2016exploring}, mobile applications \cite{ryu2006reliability} and medical instruments \cite{liljegren2006usability}).

One of the major departures from the early HCI questionnaires was the shift in focus from usability and task-oriented measures to user experience and other more aesthetic measures \cite{tractinsky1997aesthetics, hassenzahl2003attrakdiff, laugwitz2008construction, schrepp2017design}. AttrakDiff, for example, has multiple questions to evaluate user experiences on three quality dimensions: pragmatic quality, hedonic quality, and attractiveness. These variables are suggestive of aesthetic considerations as might be used in industrial design, to evaluate consumer products. 

In contrast, researchers in the communication and voice-based research space often borrow standard psychometric and relational scales from psychology and sociology; \citet{reeves1996media} for instance, argue that people interact with media and computer technology like they interact with other people, and hence they use the tools used to evaluate human interaction to measure human computer interaction. \citet{nass2005wired} go further, arguing that products that use speech and voice are perceived to have personalities,  emotions and social motivations in the way that people are. 

In light of the variance of possible perspectives on appropriate measures for speech interfaces, then, we cast a wide net in sourcing and testing multiple standards scales upon which to base our toolkit to evaluate the personality, usability and enjoyability of voice agents.




==> 03questionnaire.tex <==
\section{Questionnaire Development}
\subsection{Literature Meta-Review}
An exhaustive review of literature was conducted to establish an understanding of the most relevant scales and measures of VUIs. The review not only included canonical VUIs literature but also relevant literature from social-robot interaction and embodies voice agents. The goal was to gain an overview of research on VUIs and related domains and to identify the most important scales and measures in this domain. Based on combinations of key-words (voice interaction, social robots, affective computing, conversational interfaces, speech interfaces etc.) and a number of citations from research databases, relevant papers were collected and reviewed focusing on the goodness criteria for VUIs. Additionally a systematic review of the conference proceedings from the last five years including the conferences CHI, CSCW, AutoUI, DIS, MobileHCI and IUI. The goal of this material was to identify what evaluation methods have been applied in the most recent studies on VUIs.

\subsubsection{Paper Clusters}
We cluster the literature into five categories discussed briefly below.

\paragraph{Voice User Interface In Everyday Life}
Qualitative interviews and ethnographic work looking at in-situ use of VUIs is informative for understanding how these systems are being put in use today. Interviews have shown significant gaps between user expectations and device capabilities \cite{luger2016like}. Months long evaluations of VUIs placed in the home have studied how the device may be made accountable and embedded in multi-party interactions \cite{porcheron2018voice}. The social experience of an interaction with a VUI shows wide variation. Analysis of user reviews of the Amazon Echo and its VUI Alexa show significant divergence in user's personification of the device and the names or pronouns they choose to refer to it \cite{purington2017alexa}. Surveys of existing users of voice agents elucidates challenges with the usability of these systems that may present areas for technical improvement \cite{pyae2018investigating}. While voice user agents have existed for decades, more advanced and mainstream VUIs such as Siri, Alexa and Google Home attempt to be significantly more interactive, requiring new forms of interaction design.

\paragraph{Conversational Skills and Personality}
A large body of work in conversational analysis is being leveraged for the development of Conversational UX as a distinct design space \cite{moore2017conversational}. Conversational flow and turn taking has been explored by researchers interested in VUIs as well has in Human Robot Interaction (HRI). When interacting with limited systems, people will often modulate their own speech in response \cite{pelikan2016nao, porcheron2018voice}. The capacity for VUIs to interact in a way people find natural has implications for the devices utility to users.

\paragraph{Usability}
Comparisons of the four most popular voice assistants show that on metrics of both naturalness of interaction and usability, these systems still leave a lot to be desired \cite{lopez2017alexa}. Measures of system performance are widely varied \cite{mctear2016evaluating} and can be separated into overall system evaluations and component evaluations. An example of an overall system evaluation is the PARAdigm for DIalogue Evaluation System (PARADISE), a weighted combination of metrics which capture task success, dialog efficiency, dialog quality, and user satisfaction \cite{walker1998evaluating}. Component level evaluation is a collection of numerical metrics for the functionality of VUI technology such as word error rate for the evaluation of Automatic Speech Recognition. 

\paragraph{Joy and Engagement}
% I am a bit confused by the citations Sven put in this section
Multiple scales can be considered when evaluating a participants’ perception of VUIs. For example, a modified version of Christophel’s Trait Motivation Scale was used to measure the effects of robot behavior on student motivation \cite{szafir2012pay}. A participant’s engagement with an autonomous system can be measured by ability to recall details of a story, the perception of a robot, and any self-reported learning \cite{szafir2012pay}. Learnability and discoverability can be seen as a medium in which engagement is fostered. The learnability of a VUI is most challenging during a user’s initial encounter with it \cite{corbett2016can}. Anthropomorphic interfaces can be measured by how much spoken feedback there is within a system. Researchers \cite{qvarfordt2003role} found that people prefer more tool-like interactions but if they experienced a good alternative, would begin to prefer a more human-like interaction. The quality of engagement can be an indicator of joy that a user experiences. %(needs citation about why joy can be measured w engagement. Also unsure about how joy and engagement are related).


\paragraph{Long Term Interaction and Relationships}
VUIs can be understood as a category of relational agents, defined by Bickmore and Picard \cite{bickmore2005establishing} as ``computational artifacts designed to establish and maintain long-term social-emotional relationships with their users''. VUIs reside in users devices and their homes and have the potential to maintain interactions for extended periods of time.  Attempts have been made to explicitly design for long term companionship in interactive systems \cite{benyon2007introducing}. A VUI in a shared common space acting as a relational agent can affect the overall group dynamics of the people who interact with it \cite{lee2019hey}.

\subsubsection{Constructs}
From the literature review we identified the following constructs as critical for the
evaluation of the experience of VUIs:
\begin{itemize}
    \item Positive and negative emotions triggered by the system 
    \item User acceptance of the system
    \item The relationship between the user and the system
    \item The attitudes towards the system
    \item The personality and character conveyed by the system
    \item Companionship features of the system
    \item The perceived intelligence of the system
\end{itemize}
With an understanding of the relevant constructs for interaction with voice agents, we looked at the validated questionnaires used in our Meta-analysis.

\subsection{Questionnaire Super-Set}
We collected a set of validated measurement instruments such as scales and diagnostic tools that address various aspects of VUI evaluations. The collection includes VUI evaluation tools as well as scales from related domains such as psychology and sociology as well as industry standards.

\subsubsection{SASSI - Subject Assessment of Speech Interfaces}
The SASSI questionnaire \cite{hone2000towards} consists of 50 statements that measure the VUI system on six main factors: System Response Accuracy, Likeability, Cognitive Demand, Annoyance, Habitability and Speed. It is the most apt for VUI evaluation of any of the instruments we surveyed. However, it was developed in 2000, when speech interfaces were more focused on users providing speech input than on agents providing complex interaction and response. %We added the items of this scale with the assumption that it would compromise the backbone for the questionnaire. 
As such, it is strongly focused on usability and system performance, two factors crucially important for enjoyability with a VUI. In fact, we assume that all the other factors will provide a meaningful alteration to the items of the SASSI questionnaire emphasizing the mature technology of current VUI systems. 

\subsubsection{UTAUT Scale - Unified Theory of Acceptance of Technology}
This scale measures the acceptance of social technology such as robots or personal assistants. It is an extension of the TAM (technology acceptance model) with a focus on social factors to evaluate long-term relationships with social robots. It adds a personality dimension and can be applied to all types of social technologies in particular intelligent technologies. The inventory measures 13 constructs: anxiety, attitude toward technology, facilitating conditions, intention to use, perceived adaptiveness, perceived enjoyment, perceived ease-of-use, perceived sociability, perceived usefulness, social influence, social pressure, trust and use \cite{heerink2010assessing}.

\subsubsection{WAI - Working Alliance Inventory}
The WAI is a questionnaire developed to measure the alliance between a psychotherapist and its clients. In psychotherapy it is successfully applied since (1989). It contains 36 items to measure three fundamental constructs of productive relationships: (1) bonds, (2) goals, and (3) tasks. The development is based on content analysis Bodin’s description of the factors followed by expert and practitioner ratings. The questionnaire was used in various studies on VUI and Social Robots and contributes to the evaluation goal as the items measure the goal-driven qualities of a relationship. As VUI are mostly used for accomplishing a goal this scale may be of crucial importance\cite{horvath1989development}.

\subsubsection{RAS - Robot Anxiety Scale and NARS - Negative Attitudes towards Robots Scale}
The hypothesis of these scales are that people unconsciously interact with intelligent systems (particular anthropometric ones) in a similar manner that they would interact with people. Based on the psychological research on Communication Apprehension scales they developed RAS and NARS. Whereas NARS ask for opinions i.e. state-like attitudes, RAS ask for state-like anxiety that may be evoked by the robot. Even though both scales are better suited for profiling the user than the robots, we added their items to the superset. The reasoning was to explore if negative attitudes may correlate with system based items. Furthermore, one unexpected finding of the questionnaire was that persons with high negative attitude and anxiety toward interacting with robots tend to talk emotionally with them. The attitude seems to have an impact on emotions and as such may be an important predictor for joyful experiences with VUIs \cite{nomura2008prediction}.

\subsubsection{NEO-Five-Factor Inventory}
Personality characteristics of the VUI play a crucial role in user interactions. Commercial VUI vendors brand their VUI personalities with features representing brand values and as such it is critical to gain insight on how the user evaluates personality features. One of the most important personality questionnaires is the NEO-Five-Factor Inventory that measures five personality traits with 28 items: Neuroticism, Extraversion, Openness to
Experience, Agreeableness, Conscientiousness \cite{costa1995persons}.

\subsubsection{CSAP - Companionship Scale for Artificial Pets}
The purpose of CSAP is to measure the companionship between user and artificial pets after long term use. It is based on a literature review. The authors defined 9 key companionship factors in the literature review from research on (1) companionship with real pets, (2) Human companionship, (3) companionship features of artificial pets. As an important feature of VUI is that they are always available and companionship an indicator for retention and bond between two agents, we included this scale \cite{luh2015development}.


\subsubsection{Godspeed Scale}
Besides personality traits, most VUIs have distinctive anthropomorphic features such as gender, name, intonation and are embodied either virtually or physically. The literature review showed that these factors are of crucial importance and as such we added the items from the Godspeed scale. It contains five scales: anthropomorphism, animacy, likability, perceived intelligence and perceived safety. Each of these scales consists of a set of bi-polar dimensions \cite{bartneck2009measurement}.


\subsection{Dimension Reduction}
 After collecting all items from the standardized questionnaires above, we had a table consisting of 235 items that describe 50 scales. The first step to clean the inventory was to remove redundant items. To do so, we searched the inventory for questions that seem to be closely related but address the same content. In the second step, we removed items and scales that are not applicable or adaptable for VUI scenarios. This was particularly the case for items of inventories designed for social contexts such as WAI and NEO. Furthermore, we removed or rearranged the scale of items with the objective that all remaining items are rated by a 5-point Likert scale. The remaining 103 items were reviewed and adapted to the context of VUIs.

The reduced 103-item questionnaire super-set is still too long to be useful in most evaluation scenarios. Hence, we administer the super-questionnaire to participants following interactions with VUIs, and used Principal Component Analysis (PCA) to determine the component loadings and reduce the number of questions.
\begin{figure}[h]
    \centering
    \includegraphics[width =.9\linewidth]{voice_agents.png}
    \caption{Evaluation Setup}
    \label{fig:setup}
\end{figure}
\subsubsection{Methods} Participants (\textit{N}=13) recruited through convenience sampling were individually brought into a room containing a Google Home, an Alexa Dot, and an Apple Home Pod seen in in Figure \ref{fig:setup}. The researcher presented them with the wake word for each device and a Demo Request such as ``Hey Siri, how are you.'' Participants were asked to interact with the three systems for at least 10 minutes. A guide of possible requests and tasks was provided but the participants were instructed to be free and spontaneous in their interaction. The researcher left but monitored the interactions remotely. After 10-15 minutes (depending on the participants activity of interaction with the
system) the researcher entered the room and provided a digital version of the 103-item questionnaire with the order randomized. Participants were asked to fill out the survey and were free to continue interacting with the device as they did so.

\subsubsection{Principal Component Analysis}
We assume that many of our factors are correlated and performed principal component analysis with  direct oblim rotation. As illustrated in the scree plot in Figure \ref{fig:scree}, this results in 14 components with eigenvectors greater than one that explain more than 95\% of the total variance in our data. 

\begin{figure}[h]
    \centering
    \includegraphics[width=.9\linewidth]{scree_plot.png}
    \caption{Scree Plot}
    \label{fig:scree}
\end{figure}


In order, we labelled those components:
\begin{itemize}
    \item[-] \textit{Pleasure}: The degree to which users enjoy using the system
     \item[-] \textit{System Performance}: The degree to which the system behaves as expected and performs effectively
     \item[-] \textit{Playfulness}: The degree to which the system conveys lighthearted personality traits
     \item[-] \textit{Speed}: The efficincy of the system
     \item[-] \textit{Calm}: The degree the system is calm.
     \item[-] \textit{Trust}: The degree to which the user trusts the system
     \item[-] \textit{Dynamics}: The degree to which the system is dynamic and energetic.
     \item[-] \textit{Negative Attitudes}: The degree to which the system stimulates feelings of stress and unease in the user
     \item[-] \textit{Understanding}: The capacity for the system to interpret and adapt to interaction.
     \item[-] \textit{ Happiness}: The degree to which the system conveys is own positive or negative emotional affect. 
     \item[-] \textit{Friendliness}: The degree to which the system is perceived as affable.
     \item[-] \textit{Companionship}: The degree to which the system can be treated like a friend.
     \item[-] \textit{Usefulness}: The perceived utility of the system
     \item[-] \textit{Consistency}: The degree to which the system behaves in a predictable manner.
\end{itemize}
 . We conducted component analysis iteratively, removing components with loadings below 0.6 before conducting the PCA again.

\subsection{Synthesis}
\begin{table*}[]
\caption{The PUEVA Questionnaire Items and Scales}
\subcaption*{Personality}
\begin{tabular}{@{}p{.27\textwidth}p{.25\textwidth}p{.23\textwidth}p{.19\textwidth}@{}}
\toprule
  Conversational Skills Scale &
  Playfulness Scale &
  Happiness Scale &
  Friendliness Scale \\ \midrule
The SYSTEM is upright and honest. &
  *The SYSTEM is responsible. &
  *The SYSTEM seems depressed &
  The SYSTEM is kind. \\
The SYSTEM seems energetic.&
  The SYSTEM is foolish. &
  The SYSTEM seems cheerful &
  The SYSTEM is pleasant. \\
The SYSTEM has its own opinions. &
The SYSTEM seems self-conscious &
   &
   \\
I consider the SYSTEM a pleasant conversational partner. &
  *The SYSTEM seems assertive. &
   &
   \\ \bottomrule
   \end{tabular}
\newline
\subcaption*{Usability}
\begin{tabular}{@{}p{.27\textwidth}p{.25\textwidth}p{.23\textwidth}p{.19\textwidth}@{}}
\toprule
  System Performance Scale &
  Speed Scale &
  Understanding Scale &
  System-State Scale \\ \midrule
*The SYSTEM didn’t always do what I wanted. &
  I found the interaction with the SYSTEM to be fast. &
  The SYSTEM understands difficult conversation topics. &
  I was able to recover easily from errors. \\
*The SYSTEM didn’t always do what I expected &
  The SYSTEM always gives me an immediate response. &
  The SYSTEM adapts well to new situations. &
  The SYSTEM is well-organized. \\
A high level of concentration is required when using the SYSTEM &
   &
   &
   \\
I think I can use the SYSTEM without any help &
   &
   &
   \\ \bottomrule
      \end{tabular}
\newline
\subcaption*{Enjoyability}
\begin{tabular}{@{}p{.32\textwidth}p{.32\textwidth}p{.32\textwidth}@{}}
\toprule
  Pleasure Scale &
  Companionship Scale &
  Usefulness Scale\\ \midrule
The SYSTEM makes me happy when I talk with it. &
  Whether I am happy or sad, I want to share it with the SYSTEM. &
    I believe the time spent with the SYSTEM is not spent efficiently. 
   \\
The SYSTEM provides me with pleasurable activity. &
  The SYSTEM is like a friend who can keep me from being lonely. &
  I think the SYSTEM will help me when I need help. 
   \\
I enjoy the SYSTEM talking to me. &
   &
I found the SYSTEM to be useful. 
   \\
I find the SYSTEM fascinating. &
   &
  I am confident in the SYSTEM's ability to help me.
   \\
I like the SYSTEM. &
   &
  The SYSTEM is intelligent. 
   \\
The SYSTEM can make life more interesting &
   &
   \\ \bottomrule
\end{tabular}
\begin{tablenotes}
  \centering
  \item *Items with reversed scales
\end{tablenotes}
\label{pueva}
\end{table*}
% Here we describe the construction criteria and the final scales of the questionnnaire.  
% We run several iterations of the PCA while comparing the results with the findings from our literut review and in particular with established results from the interviews.

Using the results from the principal component analysis as inspiration rather than a decisive criteria, we developed the finalized questionnaire. To do so, we ran several iterations keeping only items with a larger loading than 0.6. Analysing and comparing the components, we constructed the final questionnaire consisting of the following changes. First we removed the \textit{Calm} and the \textit{Trust} component which had only one item each that seemed to be captured in items of the other components. We also removed the \textit{User Attitudes} component as it is beyond the scope of the questionnaire's intention. Furthermore, we renamed the \textit{Dynamics} component to \textit{Conversation Skills} after several items dropped in further iterations. Similarly, we renamed the \textit{Consistency} component to \textit{System State} after items dropped in further iterations. Lastly, a few ambiguously worded questions were removed or substituted for highly-correlated items from the structure matrix. 

The resulting questionnaire comprises 35 five-point Likert questions grouped in 11 scales as listed in Table 1. Each of the scales consists between 2 to 5 items. We assigned the scales into three categories depending of the inquiry target. Personality, for scales that assess the characteristic of the system. Usability, for scales that measure the functionality of the interactions with the system and Enjoyment, consisting of the scales that measure the experiential impact of the system. 




==> 04externalValidation.tex <==
\section{External Validation}
\begin{table*}[hbt!]
\caption{Scales and Sub-scales emerging from Interviews and Self-reports}
\label{scales}
\begin{tabular}{@{}p{.23\textwidth}p{.24\textwidth}p{.23\textwidth}p{.22\textwidth}@{}}
\toprule
Usability Issues       & Conversational Skills and Traits & Relationship Building & Enjoyment and Pleasure \\ \midrule
Dealing with errors    & Follow-up questions              & Structure of the day  & Enjoyment through play \\
Visuals and embodiment &
  Communication patterns &
  Friendship and Companionship &
  Through venting / aggression \\
System performance &
  Conversation triggers &
  Aesthetic of the voice &
  Through getting things done \\
Learnability and adaptability of the system &
  User’s self-reflection on how they communicate with the system &
  Building relationships and personality &
   \\
Knowledge of the system state and its capabilities &
  System intelligence &
  &                        \\ \bottomrule
\end{tabular}
\begin{tablenotes}
  \item *There were two additional top-level categories without sub-scales: (1) Privacy and Safety and (2) System / feature request
\end{tablenotes}
\end{table*}


To check the super-set and the PUEVA Questionnaire holistically, we collected self-reports from 41 sources. We conducted a structured questionnaire with 20 self-reported VUI users, administered over Mechanical Turk. We also conducted 18 semi-structured in-person interviews with VUI users, focusing on the three most used VUI systems: Apple’s Siri, Amazon’s Alexa and Google Assistant. The questionnaire-based self-reports consisted of seven open-ended questions about their experience with VUI systems:
\begin{enumerate}
    \item What voice agent do you use?
    \item For what purpose do you use it?
    \item Can you describe the voice agent?
    \item Tell me a surprising moment with the agent?
    \item What features or skills are you missing the most?
    \item What are positive and negative experiences with the voice agent?
    \item What would be the criteria if you buy a new voice agent?
\end{enumerate}

\subsubsection{Structured Questionnaires (\textit{N}=20)}

The structured interviews were conducted via Mechanical Turk. We recruited 20 self-reported users of common Voice User Interfaces. The users reported that they use: Amazon Alexa (9), Google Assistant (5), Apple's Siri (2), IBM Watson (1), Yandex Alisa (1), Bixbi (1). The answers were clustered based on user's answers to the questions above and analysed towards user experience issue and scales.

\subsubsection{Semi-structured Interviews (\textit{N}=18)}
The semi-structured interviews were conducted face-to-face or over the phone. The interviews were guided by the same seven questions. The interviews were between 5 to 20 minutes long. Besides the participant gender (7 female, 11 male), no personal data was collected. All interviews were recorded and transcribed by a professional transcription service. The participant used the following devices: Apple’s Siri: 8, Google Assistant: 6, Amazon Alexa: 4. Some of the participants reported that they use more than one agent. In contrast to the structured interviews, each transcript was analysed individually.

Interviews and self-reports were systematically analyzed to identify potential scales that were missing in the super-set. The goal was thereby to collect the user’s unexpected experiences with their system. The evaluation procedure consisted of three steps:
\begin{enumerate}
    \item All sources were annotated towards emerging themes. The sources were coded by the same researcher who also constructed the super-set. The focus was on unexpected findings that contributed to the pleasure and joy with the VUI.
    \item For each source the emerging themes were collected and summarized at the end of the transcripts. Each of them was classified under a top-level construct.
    \item The summaries of the emerging themes were collected and merged into a single classification of ‘potential scales’. Redundant themes were merged and the wording unified.
    \item The potential scales document was reviewed interactively and categories and themes were aligned with the wording from the super-set for better comparison.
\end{enumerate}
\subsection{Themes and Scales}
The grouping of themes from the interviews and self-reports resulted in six top-level categories and 20 potential scales which make up those top level categories. Each of these potential scales has been constructed by various related experiences reported by the participants.

==> 05discussion.tex <==
\section{Discussion}
%Interacting with a voice agent is no longer uncommon, which suggests a need for a more modern and standard approach to evaluating VUIs in order to keep up with user expectations. 
The PUEVA Inventory standardizes the process by which VUIs can be developed on the basis of personality, usability, and enjoyability. While the open-ended survey and interview of people's interactions with voice agents contained many interesting anecdotes and heartfelt feelings, they also took a lot of time to process and map to themes. We believe that the inventory design covers many of the key issues that influence judgement of voice agents. Moreover, the inventory has been tested to be understandable and easy to use. Whereas the 103-item questionnaire took up to 15 minutes to complete, the 35-item PUEVA inventory should be deployable within 5 minutes.  %The PUEVA Inventory allows for a specialized approach that delves into interactions users can have with a VUI that account for system personality and enjoyability. It takes the varied preferences of users into consideration. The habits and priorities of users are always evolving in tandem with the ever changing advances in technology.

\subsection{Reliability of the scale}
\begin{table}[]
\caption{Cronbach's Alpha for PUEVA Scales}
\begin{tabular}{ccccl}
\hline
\multicolumn{5}{c}{\textbf{Personality}}                                                                         \\ \hline
Conversational Skills Scale & Playfulness Scale   & Happiness Scale     & \multicolumn{2}{c}{Friendliness Scale} \\
0.775                       & 0.672               & 0.646               & \multicolumn{2}{c}{0.799}              \\ \hline
\multicolumn{5}{c}{\textbf{Usability}}                                                                           \\ \hline
System Performance Scale    & Speed Scale         & Understanding Scale & \multicolumn{2}{c}{System-State Scale} \\
0.412                       & 0.900               & 0.765               & \multicolumn{2}{c}{0.850}              \\ \hline
\multicolumn{5}{c}{\textbf{Enjoyability}}                                                                        \\ \hline
Pleasure Scale              & Companionship Scale & \multicolumn{3}{c}{Usefulness Scale}                         \\
0.909                       & 0.857               & \multicolumn{3}{c}{0.848}                                   
\end{tabular}
\end{table}
The PUEVA questionnaire achieves a Cronbach's alpha of 0.786, which is an ``acceptable'' degree of consistency using \citet{george2003spss}'s rule of thumb. (Cronbach's alpha remains a standard reported measure in questionnaire development, the authors acknowledge it is a flawed lower bound measure of questionnaire reliability \cite{sijtsma2009use}.) 
%For use as a design tool, the greater metric of interest for the PUEVA questionnaire is its predictive validity. We propose iterative use of PUEVA during the design stages of a Voice user agent. At each stage, regressing PUEVA scale scores on dependent variables such as interaction regularity, length, and participant physiological arousal \cite{nourbakhsh2017detecting}.

\subsection{Comparison of scale to themes from self-reports}

Our analysis of the self-report data indicates that the PUEVA scale, which is based on existing scales for evaluating voice agent interaction, covers many aspects of what users highlight as important to voice agent interaction: Dealing with errors, Communication patterns, Friendship and Companionship, Aesthetic of the Voice, Pleasure of playing with the system, and  Pleasure of getting things done.

This work also suggests some aspects for future augmentation of the PUEVA scale. Aspects which are implicitly addressed by the scales but might be more specifically interrogated are: Knowing the system state and what the system can do, Learnability and adaptability of the system, System performance,  Follow-up questions, Verbosity, Conversation triggers, System intelligence , Building relationships and personality, Privacy and Safety concerns, System / feature request. 

Some aspects from the self-reports that people care about are not yet covered by the PUEVA inventory:  Visuals and embodiment, User’s self-reflection on how they communicate with the system, Structure the day, Pleasure of venting / aggression. We believe visuals and embodiment to be particularly important. For example, if, in a car, a person asks for nearby restaurants, it is beneficial if the agent can show a listing of restaurants and relative distances, or locations on a map; these are all better than reading out each listing aloud. 

\subsection{Comparison of PUEVA to other scales} 

One of the motivations for the PUEVA scale is that many existing assessment methods for Voice User Interfaces \cite{hone2000towards} are oriented toward basic voice input operations rather than the variety of more fully fledged interactive agents increasingly at use. Leveraging these scales as a basis but including subjective measures from fields such as Human Robot Interaction (HRI) and social psychology helps us to maintain the face and construct validity of our questionnaire while expanding their usage toward modern VUI applications. As a whole, there are no existing scales like PUEVA, which seeks to evaluate how users perceive voice agents, whose interactions are becoming increasingly human-like. 

How similar is PUEVA to any of its constituent scales? This is an important question, even if we feel the PUEVA scale adds important dimensions to the overall analysis of interactive agents, as high similarity might indicate that comparisons with prior research using prior research is viable. Of all included inventories, the SASSI questionnaire seems predictably to be the most similar in terms of the structure of the scales, despite the fact that only 6 SASSI items made it into the PUEVA inventory. Almost all (i.e. 5 of the 6) SASSI items, were loading on our usability scales, particularly the System Performance Scale. The only exception is the item "The SYSTEM is pleasant" which had a high factor load on our Friendliness component. Surprisingly, none of the Annoyance items of the SASSI inventory was loading significantly on our 11 identified components. In other words, despite some overlap in questionnaire items, the PUEVA inventory measures  very different contructs than SASSI overall. 

On the whole, the PUEVA inventory emphasizes personality- and relationship-related constructs over usability- and performance-related constructs. We believe that the shift in focus was impacted by two phenomena. First and foremost, the commercial VUI systems that we used in conducting the studies that informed the PUEVA inventory questions and weights are much more mature than the system from the time of SASSI's development in 1999/2000. Secondly, the basis for constructing PUEVA consisted of a much more varied sources of questions items, including personality and relationship oriented inventories. Finally, from a methodological perspective, we did not give our participants a definitive task to perform but motivated them to "toy around" with the system at will. This focus seemed to orient the evaluation towards more positive, emotional or relation-able constructs of the source inventories, as our participants were able to explore the pleasurable and communicative qualities of the systems. Looking beyond the usability of the VUI systems, we believe that the PUEVA questionnaire helps to assess the actual relational quality of the interacting in natural language with an artificial system by covering the key aspects discussed in literature: personality, usability and enjoyability. 

\subsection{Other possibilities for extension of PUEVA} 

As we mentioned, we know the PUEVA inventory does not cover all the factors that we discovered that people care about in our interviews:  Visuals and embodiment, Users' self-reflection on how they communicate with the system, Structure the day, Pleasure of venting/aggression. We believe visuals and embodiment to be particularly important factors, which are currently not addressed by our inventory. For example, if, in a car, a person asks for nearby restaurants, it is beneficial if the agent can show a listing of restaurants and relative distances, or locations on a map; these are all better than reading out each listing aloud. 

While PUEVA was developed for immediate contextual feedback on design, we feel there are opportunities to extend the scales to address longitudinal use. The playfulness of a brief interaction may become annoying with extended use. To that end, we acknowledge the need for additional items and/or additional scales to capture factors pertaining to longer-term interaction and usage.

% Limitation of the apporach: It's a first step in constructing a tool that focusses on inter-personal and emotional aspects of the VUIs. 
% How can we employ and use PUEVA? Longitunial, in design etc. 

% Next steps: evaluation of the PUEVA qeustionnaire in various settings. 

% The utility of a voice agent to a user extends beyond the practicality of a VUI. Voice agents have become an extension of the home and with it comes the need to evaluate the pleasurable aspects of VUIs. The PUEVA Inventory was developed through a comprehensive literature review of canonical and seminal research contributions, VUI papers from HCI conferences, and validated scales that not only included VUI evaluation tools, but also scales from related areas such as psychology and sociology. We then created a superset of questions based on standardized evaluation instruments used in academia and industry research. A dimension reduction was necessary to reduce the questionnaire from 103 items. After conducting a principal component analysis on the data we collected, we generated the current PUEVA Inventory. Evaluating voice agents not only on their pragmatic applications but also on their personality and enjoyability is important when keeping up with user expectations. We anticipate that this will act as a guideline in designing prospective VUIs.

==> 06conclusion.tex <==
\section{Conclusion}
 The main contribution of this work is a research and assessment instrument, the PUEVA Inventory, designed to aid in evaluating pleasurable experiences of voice user interface by novice users based on short-term use. This inventory was built on an exhaustive list of scales and measures that can be used to evaluate relevant HCI systems, and then validated against unstructured self-report data about people experiences with voice interfaces. We believe this instrument to be particularly useful for current-day voice interactions, which have greater focus on personality and enjoyment than the more basic task-oriented voice interfaces of old. With an increasing number of VUIs emerging onto the market, we hope researchers will use the PUEVA Inventory to make friendlier, more approachable and more enjoyable interfaces for us all to use.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix


==> abstract.tex <==
The proliferation of voice agents in consumer devices requires new tools for evaluating these systems beyond their technical functionality. This paper presents a toolkit for the evaluation of Voice User Interfaces (VUIs) with the intention of measuring the crucial factors of subjective enjoyment in the user experience. The PUEVA toolkit was constructed using a meta-analysis of existing literature, structured (\textit{N}=20) and  semi-structured (\textit{N}=18) interviews and a within subjects lab study. The resulting questionnaire contains 35 items that represent 12 scales in three categories: (1) \textit{Personality} (2) \textit{Usability} and (3) \textit{Enjoyability}. The PUEVA Toolkit moves us towards the capacity to evaluate and compare subjective, joyful experiences in between-subject as well as within-subject research designs.

==> lbr/104externalValidation.tex <==
\section{External Validation}
\begin{table*}[hbt!]
\caption{Scales and Sub-scales emerging from Interviews and Self-reports}
\label{scales}
\begin{tabular}{@{}p{.23\textwidth}p{.24\textwidth}p{.23\textwidth}p{.22\textwidth}@{}}
\toprule
Usability Issues       & Conversational Skills and Traits & Relationship Building & Enjoyment and Pleasure \\ \midrule
Dealing with errors    & Follow-up questions              & Structure of the day  & Enjoyment through play \\
Visuals and embodiment &
  Communication patterns &
  Friendship and Companionship &
  Through venting / aggression \\
System performance &
  Conversation triggers &
  Aesthetic of the voice &
  Through getting things done \\
Learnability and adaptability of the system &
  User’s self-reflection on how they communicate with the system &
  Building relationships and personality &
   \\
Knowledge of the system state and its capabilities &
  System intelligence &
  &                        \\ \bottomrule
\end{tabular}
\begin{tablenotes}
  \item *There were two additional top-level categories without sub-scales: (1) Privacy and Safety and (2) System / feature request
\end{tablenotes}
\end{table*}


To check the super-set and the PUEVA Questionnaire holistically, we collected self-reports from 41 sources. We conducted a structured questionnaire with 20 self-reported VUI users, administered over Mechanical Turk. We also conducted 18 semi-structured in-person interviews with VUI users, focusing on the three most used VUI systems: Apple’s Siri, Amazon’s Alexa and Google Assistant. The questionnaire-based self-reports consisted of seven open-ended questions about their experience with VUI systems:
\begin{enumerate}
    \item What voice agent do you use?
    \item For what purpose do you use it?
    \item Can you describe the voice agent?
    \item Tell me a surprising moment with the agent?
    \item What features or skills are you missing the most?
    \item What are positive and negative experiences with the voice agent?
    \item What would be the criteria if you buy a new voice agent?
\end{enumerate}

\subsubsection{Structured Questionnaires (\textit{N}=20)}

The structured interviews were conducted via Mechanical Turk. We recruited 20 self-reported users of common Voice User Interfaces. The users reported that they use: Amazon Alexa (9), Google Assistant (5), Apple's Siri (2), IBM Watson (1), Yandex Alisa (1), Bixbi (1). The answers were clustered based on user's answers to the questions above and analysed towards user experience issue and scales.

\subsubsection{Semi-structured Interviews (\textit{N}=18)}
The semi-structured interviews were conducted face-to-face or over the phone. The interviews were guided by the same seven questions. The interviews were between 5 to 20 minutes long. Besides the participant gender (7 female, 11 male), no personal data was collected. All interviews were recorded and transcribed by a professional transcription service. The participant used the following devices: Apple’s Siri: 8, Google Assistant: 6, Amazon Alexa: 4. Some of the participants reported that they use more than one agent. In contrast to the structured interviews, each transcript was analysed individually.

Interviews and self-reports were systematically analyzed to identify potential scales that were missing in the super-set. The goal was thereby to collect the user’s unexpected experiences with their system. The evaluation procedure consisted of three steps:
\begin{enumerate}
    \item All sources were annotated towards emerging themes. The sources were coded by the same researcher who also constructed the super-set. The focus was on unexpected findings that contributed to the pleasure and joy with the VUI.
    \item For each source the emerging themes were collected and summarized at the end of the transcripts. Each of them was classified under a top-level construct.
    \item The summaries of the emerging themes were collected and merged into a single classification of ‘potential scales’. Redundant themes were merged and the wording unified.
    \item The potential scales document was reviewed interactively and categories and themes were aligned with the wording from the super-set for better comparison.
\end{enumerate}
\subsection{Themes and Scales}
The grouping of themes from the interviews and self-reports resulted in six top-level categories and 20 potential scales which make up those top level categories. Each of these potential scales has been constructed by various related experiences reported by the participants.
